Efficient Replay Memory Architectures in Multi-Agent Reinforcement Learning for Traffic Congestion Control

Episodic control, inspired by the role of episodic memory in the human brain, has been shown to improve the sample inefficiency of model-free reinforcement learning by reusing high-return past experiences. However, the memory growth of episodic control is undesirable in large-scale multi-agent problems such as vehicle traffic management. This paper proposes a novel replay memory architecture called Dual-Memory Integrated Learning, to augment to multi-agent reinforcement learning methods for congestion control via adaptive light signal scheduling. Our dual-memory architecture mimics two core capabilities of human decision-making. First, it relies on diverse types of memory--semantic and episodic, short-term and long-term--in order to remember high-return states that occur often in the network and filter out states that don't. Second, it employs equivalence classes to group together similar state-action pairs and that can be controlled using the same action (i.e., light signal sequence). Theoretical analyses establish memory growth bounds, and simulation experiments on several intersection networks showcase improved congestion performance (e.g., vehicle throughput) from our method.

==> icmlreview.tex <==
ToDo:

* Consistent terminologies: 
\begin{itemize}
    \item The SARSA Agent was interchangeably called the Memoryless Agent because it relies just on the Q-table and not at all on the dual memory architecture we proposed. [DONE]

    \item We also used the term replay buffer and Q-table interchangeably.
    (difference between replay buffer vs q table in literature.)

    \item In our experiments (Table 1), the simple agent refers to the agent with a simple equivalence class which only utilizes shift invariance. The complex agent refers to the one that utilizes all three invariances and symmetries described in Section 4.1. The distinction between these models is mentioned at the start of Section 6.4, but we agree the language is a bit confusing when looking at Figure 1 by itself. [DONE]
\end{itemize}
We acknowledge the confusion in these terminologies, and will modify the next draft to consistently use “SARSA agent” and “Q-table” throughout. 

* Add description of Q-learning agent: Sutton and Barto’s "Reinforcement Learning". [DONE]

% * Justification for memory component: 
% % \begin{itemize}
%     % \item The dual memory architecture...was built in a modular way mostly to have better control over the functionality of the memories and how they interact with each other. This remark will be added to the paper for additional clarity.

%     % The separation into two memories, short-term and long-term, was also done to further reduce memory consumption. Essentially, the short-term memory filters out (and forgets) states that do not repeat as often in the environment; there is no point in long-term remembrance for states that happen rarely.
% % \end{itemize}

% * Small remark about Hyperparameter tuning: Our calculations provide additional constraints on the hyperparameters of our architectures. This allows us to set upper and lower bounds on these parameters and also only apply the architecture to applications where it would be beneficial (e.g., bounds on the size of action space, and bounds of frequency of updates). 
% We hope that additional clarity can be achieved after adding the training process description of the SARSA agent in the Appendix (also described in our answer to #1 above). 
% We chose the hyperparameters based on our observations and experiments, these parameters were kept consistent across all agents to be able to compare the architectures meaningfully. We opted to not perform more rigorous hyperparameter tuning of the agents with methods such as random-forest search, as these parameters are environment and application-sensitive, especially for the proposed memory architecture, and take away from the general behavioral comparison of the agents. It is, however, an avenue of future work we plan to explore.

% * More details on simulations experiment: A dummy SARSA agent is trained offline for 300 simulation seconds of incoming vehicles, modeled as homogeneous Poisson processes. The Q-table from this SARSA agent is then fed into both simple and complex dual memory agents as well as our baseline SARSA agent. We do this for continuous comparison: all agents start from the same prior knowledge. Furthermore, the dummy SARSA agent is simply used to accumulate prior knowledge of the system, while the baseline SARSA agent is actually used to benchmark our proposed simple and complex dual memory agents.  We did not add any distinct operations behind creating the Q-table for both the dummy and baseline SARSA agents. Both agents also perform the usual SARSA update Q(S_t , A_t) <- Q(S_t , A_t) + alpha[ R_{t+1}+ gamma*Q(S_{t+1}, A_{t+1}) − Q(S_t , A_t)] (Sutton and Barto), and also fetch the best state-action pair when not exploring.

* average vs. sum multiagent RL distinction: The direct sum and the averaging of the Q-function differ only in scale. The reason we were using the average was that in our memory-central unit architecture, there is information passing between memories (which stores the individual Q-function) and the central unit that stores the aggregated Q-function. If the direct sum is used for the aggregation method, then the centralized Q-function will have a different scale from the individual Q-function. In that case, the centralized Q-function cannot be passed back to memories due to the different scaling. In future drafts, we will revise Remark 3.2 to add this additional clarification.

* some additional insights into the reduced performance of communication layer experiments: From what we observed, the introduction of the communication layer often increased waiting times in the 3x3 grid setting with the default reward function, as seen in Figure 4. However, as shown in Table 3, this behavior was not seen with the other two reward functions, which suggests that reward design should also be considered carefully. Figure 5 and lines 431-439 showcase the reduction in memory growth due to communication. Our claim comes from these observations. Several references in the literature (e.g., [arXiv:2011.09533]) suggest that for some RL tasks, dependent MARL agents perform worse than independent MARL agents. Since the communication introduces further dependency among agents, we might also expect a decrease in performance. The dependency among agents, facilitated through information sharing back-and-forth between memories and a central unit via communication, forces the agents to exhibit similar Q-values for their control task even if some actions are not optimal for some agents. This phenomenon might lead to a problem called "relative overgeneralization", where the solution converges to a suboptimal joint action.

* Grammatical commments from Reviewer rDBd. [DONE.]

* Extra experiments: Our results demonstrate that the performance already scales well from the 1x1 intersection to the 3x3 grid network. We also observed similar trends of performance improvement on larger grid sizes such as 5x5; in the next draft, we can complete the 5x5 experiment and add some comparisons with the other environments. Compressing the state-action spaces through equivalence classes should also help in higher dimensional state-action spaces, and more complex embeddings (similarity metrics, i.e., what determines “equivalence”) respective to application can be employed to achieve a reduction in memory sizes.


==> sections/prose/introduction_old.tex <==
Many deep reinforcement learning (DRL) methods for control tasks are still hindered by \textit{sample inefficiency}, often needing a significant amount of training data to learn a task that a human could learn from fewer exposures~\cite{mnih_human-level_2015, haarnoja_soft_2018}. 
\textit{Memory}, then, becomes an important aspect of RL to effectively store past experiences while exploring the environment.
A common way of implementing memory is through experience replay buffers~\cite{fedus20a}, which store past states and rewards to train the agent network.
Another method is neural episodic control~\cite{pritzel17}, which implements a differentiable neural dictionary (DND), whose differentiability allows for end-to-end learning to be achieved, unlike the replay buffer, which is more like a table augmented to the training procedure for querying and inputting.

However, most memory tables (e.g., replay buffers, DNDs) are structured such that every new experience encountered is stored as a new entry, potentially leading to large memory growth.
A rapidly growing memory table is undesirable in applications such as large-scale network control problems, and also unnecessary because there may exist natural spatial structures and temporal repetition that can be leveraged. 
For example, in vehicle traffic flow over metropolitan intersection networks, spatial symmetries arise from the grid-like topology, while temporal symmetries arise from human routine (e.g., every weekday, people commute to work every morning and evening).
Recent work in incorporating symmetry inductive biases into conventional neural networks has demonstrated the powerful idea of encoding rotation symmetry~\cite{cohen16} or permutation invariance~\cite{battaglia18} to reduce the number of parameters that need to be trained and improve performance.

This paper proposes \textit{dual-memory integrated learning}, a novel memory architecture to include in multiagent reinforcement learning (MARL) algorithms for efficient control and decision-making over large-scale networks.
We are largely motivated by the efficiency of human decision-making, which effectively uses \textit{different combinations} of memory instead of relying on just one type.
% For the concreteness of the presentation, we focus specifically on the application of vehicle traffic congestion control in an urban intersection grid network by managing the light signals.
In vehicle traffic congestion control, previous work~\cite{pmlr-v211-han23a} has demonstrated that learning patterns can prevent the controller synthesis procedure from spending unnecessary time and energy redundantly computing light signals for scenarios that have been previously observed.
The pattern learning was largely implemented based on episodic memory~\cite{gershman_reinforcement_2017}; in contrast to semantic memory, which stores only the statistical summaries of event trajectories, episodic memory saves episodic traces along with their returns.
This work differs from~\cite{pmlr-v211-han23a} by striving to improve the table's rate of growth in two primary ways.
First, we develop a two-step short-term and long-term memory approach for a more robust way of identifying which patterns occur frequently enough in the system to warrant permanent storage in memory.
Second, we borrow ideas from group-equivariance to define the symmetry relations to form equivalence classes of patterns such that each equivalence class is assigned to a single action sequence.
% Our approach is validated through a series of experiments... TBD.

% However, solely relying on semantic memory is inefficient as some events happen infrequently, causing inferences on those states to be inaccurate. 
% These episodic traces are then utilized for future references when the agent is facing a similar state with the saved experiences. 
% Such a method applies to environments with huge state space such as traffic control where the possible vehicle numbers coming from each direction are huge. 

Our paper is organized as follows.
We begin with a brief review of relevant background in~\sec{background}, such as MARL, memory in RL, and equivariance.
The main problem formulation is described in~\sec{problem_formulation}.
Our main contributions--the dual-memory integrated learning framework, equivalence classes and other constituents--are detailed in~\sec{memory}.
The remaining sections compare the performance of our dual-memory integrated learning framework against state-of-the-art baselines, with theoretical analyses in~\sec{analysis} and simulation experiments in~\sec{experiments}.
We conclude the paper in~\sec{conclusion}.

